The Finite State MAC with Cooperative Encoders and Delayed CSI

In this paper, we consider the finite-state multiple access channel (MAC) with partially cooperative encoders and delayed channel state information (CSI). Here partial cooperation refers to the communication between the encoders via finite-capacity links. The channel states are assumed to be governed by a Markov process. Full CSI is assumed at the receiver, while at the transmitters, only delayed CSI is available. The capacity region of this channel model is derived by first solving the case of the finite-state MAC with a common message. Achievability for the latter case is established using the notion of strategies, however, we show that optimal codes can be constructed directly over the input alphabet. This results in a single codebook construction that is then leveraged to apply simultaneous joint decoding. Simultaneous decoding is crucial here because it circumvents the need to rely on the capacity region's corner points, a task that becomes increasingly cumbersome with the growth in the number of messages to be sent. The common message result is then used to derive the capacity region for the case with partially cooperating encoders. Next, we apply this general result to the special case of the Gaussian vector MAC with diagonal channel transfer matrices, which is suitable for modeling, e.g., orthogonal frequency division multiplexing (OFDM)-based communication systems. The capacity region of the Gaussian channel is presented in terms of a convex optimization problem that can be solved efficiently using numerical tools. The region is derived by first presenting an outer bound on the general capacity region and then suggesting a specific input distribution that achieves this bound. Finally, numerical results are provided that give valuable insight into the practical implications of optimally using conferencing to maximize the transmission rates.

==> mnsymbol/README <==
MnSymbol is a symbol font designed to be used in conjunction with Adobe
MinionPro.

All files in this archive are in the public domain.

WARNING
=======

This version includes a bugfix that causes incompatibilities with
previous versions. The symbols

  \...harpoonup and \...harpoondown

are now called

  \...harpoonccw and \...harpooncw

(This was needed for compatibility with amsfonts.sty.)

INSTALLATION
============

To install the fonts:

(0) If you have already a version of MnSymbol installed, delete the old
TFM and PK files.

(1) Run

  $ cd tex
  $ latex MnSymbol.ins

and copy the resulting file MnSymbol.sty to

   .../texmf/tex/latex/MnSymbol/MnSymbol.sty

(2) Copy all files in the "source" directory into the directory

   .../texmf/fonts/source/public/MnSymbol/

(3) Copy the documentation (MnSymbol.ps, MnSymbol.pdf, README) into the
directory

   .../texmf/doc/latex/MnSymbol/

(4) To install the PostScript fonts (courtesy of Michael Zedler) copy

  o enc/MnSymbol.map into .../texmf/fonts/map/dvips/MnSymbol
  o enc/*.enc        into .../texmf/fonts/enc/dvips/MnSymbol
  o pfb/*.pfb        into .../texmf/fonts/type1/public/MnSymbol

(These fonts are not strictly necessary but recommended.)

(5) You can copy the files in the "tfm" directory to

   .../texmf/fonts/tfm/public/MnSymbol

This is optional since these files can be generated automatically.
But it saves some time.

(6) Regenerate the file database:

  $ mktexlsr

If you installed the PostScript fonts you also need to run updmap or
updmap-sys to make them available:

  $ updmap-sys --enable MixedMap MnSymbol.map

(7) Happy TeXing.

Achim Blumensath

